Factcheck-Bench: Fine-Grained Evaluation Benchmark for Automatic Fact-checkers

The increased use of large language models (LLMs) across a variety of real-world applications calls for mechanisms to verify the factual accuracy of their outputs. In this work, we present a holistic end-to-end solution for annotating the factuality of LLM-generated responses, which encompasses a multi-stage annotation scheme designed to yield detailed labels concerning the verifiability and factual inconsistencies found in LLM outputs. We further construct an open-domain document-level factuality benchmark in three-level granularity: claim, sentence and document, aiming to facilitate the evaluation of automatic fact-checking systems. Preliminary experiments show that FacTool, FactScore and Perplexity.ai are struggling to identify false claims, with the best F1=0.63 by this annotation solution based on GPT-4. Annotation tool, benchmark and code are available at https://github.com/yuxiaw/Factcheck-GPT.

==> section/feedback.tex <==
even though there was work on reducing halucinatioons (incl. Nico's work), but they will remain, so we still need checking.

- previous work:
                - fact-checking a claim (could be complex sometimes, multi-hop, but still a sentence)
                - fake news: document, but not individual claims
                - entire website: e.g., can I trust Aljazeera

- In the age of LLMs, we need a different approach: chekc every single claim. This requires check-worthiness (what to check), understanding context, checking every claim, potentially correcting claims, and producing a new version of the text with the corrections.

- Withe the emergence of LLMs, there have been approaches that started looking into checking LLM generated text. However, they were not end-to-end, and only looked into some (subset) of these problems. In contrast, here we propose a comprehensive end-to-end solution.

- why end-to-end: 
                - maybe inter-dependencies

Our work is applicable even for human-written text, not just for LLMs, but it is motivated by LLMs.

Move the figure to page 2: refer to it to explain the terms that Iryan had a problem it


